GeoGPT4V: Towards Geometric Multi-modal Large Language Models with Geometric Image Generation

Large language models have seen widespread adoption in math problem-solving. However, in geometry problems that usually require visual aids for better understanding, even the most advanced multi-modal models currently still face challenges in effectively using image information. High-quality data is crucial for enhancing the geometric capabilities of multi-modal models, yet existing open-source datasets and related efforts are either too challenging for direct model learning or suffer from misalignment between text and images. To overcome this issue, we introduce a novel pipeline that leverages GPT-4 and GPT-4V to generate relatively basic geometry problems with aligned text and images, facilitating model learning. We have produced a dataset of 4.9K geometry problems and combined it with 19K open-source data to form our GeoGPT4V dataset. Experimental results demonstrate that the GeoGPT4V dataset significantly improves the geometry performance of various models on the MathVista and MathVision benchmarks. The code is available at https://github.com/Lanyu0303/GeoGPT4V_Project

==> figure/data_ann_difficulty.tex <==
\begin{figure}[htbp]

\includegraphics[width=0.4\textwidth]{images/difficulty.pdf}
\caption{\textbf{The proportion of difficulty in the generated data compared to the original data.}
``Easier'' represents that the generated data is easier than the original data.
``Harder'' represents that the generated data is harder than the original data.
``Equal'' represents that the generated and original data have the same difficulty level.
}
\label{fig:data_difficulty}
\end{figure}

==> figure/data_ann_matching.tex <==
\begin{figure}[htbp]

\includegraphics[width=0.45\textwidth]{images/image_text_matching.pdf}
\caption{\textbf{The average image-text matching scores for the three types of data.}
}
\label{fig:data_matching}
\end{figure}
